Approximating Discrimination Within Models When Faced With Several Non-Binary Sensitive Attributes

Discrimination mitigation within machine learning (ML) models could be complicated because multiple factors may be interwoven hierarchically and historically. Yet few existing fairness measures can capture the discrimination level within ML models in the face of multiple sensitive attributes (SAs). To bridge this gap, we propose a fairness measure based on distances between sets from a manifold perspective, named as 'Harmonic Fairness measure via Manifolds (HFM)' with two optional versions, which can deal with a fine-grained discrimination evaluation for several SAs of multiple values. Because directly computing HFM may be costly, to accelerate its subprocedure -- the computation of distances of sets, we further propose two approximation algorithms named 'Approximation of distance between sets for one sensitive attribute with multiple values (ApproxDist)' and 'Approximation of extended distance between sets for several sensitive attributes with multiple values (ExtendDist)' to respectively resolve bias evaluation of one single SA with multiple values and that of several SAs with multiple values. Moreover, we provide an algorithmic effectiveness analysis for ApproxDist under certain assumptions to explain how well it could work. The empirical results demonstrate that our proposed fairness measure HFM is valid and approximation algorithms (i.e. ApproxDist and ExtendDist) are effective and efficient.

==> main_prefix.tex <==
%%
%% This is the prefix file tailored to ACM Publishing Systems
%% List of accepted LaTeX pkgs: https://authors.acm.org/proceedings/production-information/accepted-latex-packages
%%




\def\ie{i.e.}% ,}
\def\eg{e.g.}% ,}
\def\aka{aka.}
\def\etc{etc.}
\def\etal{\emph{et al.}}
\def\wrt{w.r.t.}% with respect to
\def\iff{iff}% if and only if
% \def\TODO{\textcolor{red}{TODO:}}
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}




\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \newcommand{\topelement}[1]{\footnotesize{#1}}
\newcommand{\topelement}[1]{\scriptsize{#1}}

% ... independent symbol
\newcommand\indep{\protect\mathpalette{\protect\independent}{\perp}}
\def\independent#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand\nindep{\centernot\indep}

% \newcommand{\defineq}{\smash{\overset{\text{def}}{=}}}
% \newcommand{\defineq}{:=}
\newcommand{\defineq}{\triangleq}

% \def\xneg{\mathop{\bm{x}^\prime}}% \bar{\bm{x}}
\def\xneg{\mathop{\breve{\bm{x}}}}
\def\xpos{\mathop{\bm{a}}}
\def\xqtb{\mathop{\tilde{\bm{a}}}}

% probP, justY/Z/X
\def\probP{\mathbb{P}}
% \def\justX{\bm{x}}
% \def\justA{\bm{a}}
% \def\justY{y}
% \def\justZ{\hat{y}}
\def\insx{\bm{x}}
\def\insy{\hat{y}}

% \def\vecw{\mathbf{w}}
\def\vecw{\bm{w}}

% \def\newy{\bar{y}}
% \def\newy{\tilda{y}}
\def\newy{\ddot{y}}% it has two (different) meanings
% \def\newy{\dot{y}}
\def\comp{\mathcal{O}}


% \def\fairX{\mathsf{x}}
% \def\fairA{\mathsf{a}}
% \def\fairY{\mathsf{y}}
% \def\fairZ{\hat{\mathsf{y}}}
% \def\fairX{\mathsf{X}}
% \def\fairA{\mathsf{A}}
% \def\fairY{\mathsf{Y}}
% \def\fairZ{\hat{\mathsf{Y}}}

\def\justX{\mathsf{X}}
\def\justA{\mathsf{A}}
\def\justY{\mathsf{Y}}
\def\justZ{\hat{\mathsf{Y}}}
\def\justR{\mathsf{R}}
% \def\probP{\mathbb{P}}
% \newcommand{\propP}[1]{\mathbb{P}(#1)}
\newcommand{\propP}[1]{\mathbb{P}\{#1\}}

\def\newDist{\mathbf{D}}% \mathrm{D}}
\def\newdist{\mathbf{d}}
\def\newFist{\mathbf{D}_f}
% \def\newfist{\mathbf{d}_f}
\def\newfist{\mathbf{df}}

% \def\newdist{\mathbf{d}}
% \def\newfist{\mathbf{df}}
\newcommand{\extDist}[1]{\mathbf{D}_{\cdot,\bm{a}}^\text{#1}(S,a_i)}
\newcommand{\extEist}[1]{\mathbf{D}_{\cdot,\bm{a}}^\text{#1}(S)}
\newcommand{\extBist}{\mathbf{D}_\cdot(S_1,\bar{S}_1)}
% \newcommand{\extprev}{\mathbf{d}( (\breve{\bm{x}},\ddot{y}),(\breve{\bm{x}}',\ddot{y}') )}
% \newcommand{\extprev}{\mathbf{d}\big( (\breve{\bm{x}},\ddot{y}),(\breve{\bm{x}}',\ddot{y}') \big)}
\newcommand{\extprev}[1]{\mathbf{d}\big( (\breve{\bm{x}},{#1}),(\breve{\bm{x}}',{#1}') \big)}
% \newcommand{\extDnew}[1]{\mathbf{}}
% \newcommand{\extFist}[]{}
% \def\extDbin{\mathbf{D}_\cdot(S_1,\bar{S}_1)}


% \def\illusDist{distance measure for one sensitive attribute}
% \def\illusEist{distance measure for sensitive attributes}
\def\illusDist{distance for one sensitive attribute}
\def\illusEist{distance for sensitive attributes}

% \def\newDsM{\mathbf{D}_{\bm{a}_i}}
% \def\newFsM{\mathbf{D}_{f,\bm{a}_i}}
% \def\newDMs{\mathbf{D}_{\bm{a}}}
% \def\newFMs{\mathbf{D}_{f,\bm{a}}}
% \def\newDMi{\mathbf{D}_{\bm{a}_i}}
% \def\newFMi{\mathbf{D}_{f,\bm{a}_i}}

% \def\newDsM{\mathbf{D}_{\bm{a}}}
% \def\newFsM{\mathbf{D}_{f,\bm{a}}}
% % \def\newDiM{\mathbf{D}_{\bm{a}_i}}
% % \def\newFiM{\mathbf{D}_{f,\bm{a}_i}}
% \newcommand{\newDiM}[1]{\newDsM^\text{#1}(S,\bm{a}_i)}
% \newcommand{\newFiM}[1]{\newFsM^\text{#1}(S,\bm{a}_i)}

% \newcommand{\newDsM}[1]{\mathbf{D}_{\bm{a}}^\text{#1}}
% \newcommand{\newFsM}[1]{\mathbf{D}_{f,\bm{a}}^\text{#1}}
% \newcommand{\newDiM}[2]{\newDsM{#1}(S,\bm{a}_{#2})}
% \newcommand{\newFiM}[2]{\newFsM{#1}(S,\bm{a}_{#2})}
\newcommand\newDsM{\mathbf{D}_{\bm{a}}}
\newcommand\newFsM{\mathbf{D}_{f,\bm{a}}}
\newcommand{\newDiM}[2]{\newDsM^\text{#1}(S,a_{#2})}% \bm{a}_{#2}
\newcommand{\newFiM}[2]{\newFsM^\text{#1}(S,a_{#2})}% \bm{a}_{#2}
\def\newDMb{\overline{\mathbf{D}}_{\bm{a}}}
\def\newFMb{\overline{\mathbf{D}}_{f,\bm{a}}}




% \prop df % prpsl, prpsd, ppsd (proposal, proposed
% \def\ppsdisfull{harmonic fairness measure via manifolds}
\def\ppsdisfull{Harmonic Fairness measure via Manifolds}
% \def\ppsdisfull{Harmonic fairness measure via manifolds}
\def\ppsdisabbr{\emph{HFM}}
% \def\ppsalgfull{Approximation of distance between sets}
% \def\ppsalgabbr{\texttt{ApproxDist}}%\emph}
% \def\ppsalgabbr{\emph{ApproxDist}}
\def\ppssubfull{Acceleration sub-procedure}% in approximation}
% \def\ppssubabbr{\texttt{AcceleDist}}%\emph}
\def\ppssubabbr{\emph{AcceleDist}}
% \def\ppssuperfull{Extended distance for multiple sensitive attributes with multiple values}
% \def\ppssuperfull{Approximation of extended distance between sets for several sensitive attributes with multiple values}
% \def\ppssuperfull{Approximation of extended distance between sets for multiple sensitive attributes with multiple values}
% \def\ppssuperabbr{\emph{ExtendDist}}
\def\ppsalgfull{Approximation of distance between sets for one sensitive attribute with multiple values}
\def\ppsalgabbr{\emph{ApproxDist}}

\def\ppsuperfull{Approximation of extended distance between sets for several sensitive attributes with multiple values}
\def\ppsuperabbr{\emph{ExtendDist}}
% \def\extDistAlt{\mathbf{D}_\mathbf{a}(S,a_i)}
% \def\extEistAlt{\mathbf{D}_\mathbf{a}(S)}
\newcommand{\extDistAlt}[1]{\mathbf{D}_\mathbf{a}^\text{#1}(S,a_i)}
\newcommand{\extEistAlt}[1]{\mathbf{D}_\mathbf{a}^\text{#1}(S)}
\newcommand{\extBistAlt}[1]{\mathbf{D}_{#1}(S_1,\bar{S}_1)}

%%




% \iffalse%
\newcommand{\topcaption}[1]{% 
  % \setlength{\abovecaptionskip}{0pt}% 
  % \setlength{\belowcaptionskip}{2pt}% 
  % \vspace{-.35cm}\caption{#1}}
  \vspace{-.25cm}\caption{#1}}
\newcommand{\topcentering}{%
  \centering % 图片全局居中
  % \vspace{-.35cm} % 设置与上面正文的距离
  % \subfigtopskip=2pt % 设置子图与上面正文或别的内容的距离
  % \subfigbottomskip=2pt % 设置第二行子图与第一行子图的距离，即下面的头与上面的脚的距离
  % \subfigcapskip=-3.4pt % 设置子图与子标题之间的距离
  \subfigtopskip=1pt %
  \subfigbottomskip=1pt %
  \subfigcapskip=-2.9pt %
}
\newcommand{\topequation}{%
  % \setlength\abovedisplayskip{3pt}% shrink space
  % \setlength\belowdisplayskip{3pt}%
  \setlength\abovedisplayskip{2pt}%
  \setlength\belowdisplayskip{2pt}%
}
\newcommand{\toptabcol}{%
  % \renewcommand\tabcolsep{1.7pt}%
  \renewcommand\tabcolsep{2.7pt}% 3.4pt}
}
\newcommand{\topitemize}{%
  % \setlength\itemsep{-.3em}%
  % \setlength\itemsep{-.2em}%
  \setlength\itemsep{0em}
  \setlength{\parsep}{0pt}
  \setlength{\parskip}{0pt}
}
% \newcommand{\topelement}[1]{%
%   \footnotesize{#1}%
% }
% \fi%
